FusedRF: Fusing Multiple Radiance Fields

Radiance Fields (RFs) have shown great potential to represent scenes from casually captured discrete views. Compositing parts or whole of multiple captured scenes could greatly interest several XR applications. Prior works can generate new views of such scenes by tracing each scene in parallel. This increases the render times and memory requirements with the number of components. In this work, we provide a method to create a single, compact, fused RF representation for a scene composited using multiple RFs. The fused RF has the same render times and memory utilizations as a single RF. Our method distills information from multiple teacher RFs into a single student RF while also facilitating further manipulations like addition and deletion into the fused representation.

==> src/figures/plots.tex <==
% \begin{figure}[htbp]
%   \centering
%   \begin{subfigure}{\linewidth}
%     \includegraphics[width=\linewidth]{src/images/plot1.png}
%     \label{fig:sub1}
%   \end{subfigure}
  
%   \begin{subfigure}{\linewidth}
%     \includegraphics[width=\linewidth]{src/images/plot2.png}
%     \label{fig:sub2}
%   \end{subfigure}
%   \caption{Have to explain this.}
%   \label{fig:my_figure}
% \end{figure}
